Locate 3D: Real-World Object Localization via Self-Supervised Learning in 3D

We present LOCATE 3D, a model for localizing objects in 3D scenes from referring expressions like "the small coffee table between the sofa and the lamp." LOCATE 3D sets a new state-of-the-art on standard referential grounding benchmarks and showcases robust generalization capabilities. Notably, LOCATE 3D operates directly on sensor observation streams (posed RGB-D frames), enabling real-world deployment on robots and AR devices. Key to our approach is 3D-JEPA, a novel self-supervised learning (SSL) algorithm applicable to sensor point clouds. It takes as input a 3D pointcloud featurized using 2D foundation models (CLIP, DINO). Subsequently, masked prediction in latent space is employed as a pretext task to aid the self-supervised learning of contextualized pointcloud features. Once trained, the 3D-JEPA encoder is finetuned alongside a language-conditioned decoder to jointly predict 3D masks and bounding boxes. Additionally, we introduce LOCATE 3D DATASET, a new dataset for 3D referential grounding, spanning multiple capture setups with over 130K annotations. This enables a systematic study of generalization capabilities as well as a stronger model.

==> sections/abstract.tex <==
% We present LocateX, a model to localize an object in 3D from its textual referring expression (e.g. ``chair near entryway door''). It can directly operate on sensor observation streams (RGBD, camera pose, intrinsics), making it suitable for applications in robotics and smart glasses. This is enabled through the development of 3D-JEPA, a novel self-supervised learning algorithm (SSL) applicable to sensor point clouds. It operates by first lifting features from 2D foundation models like CLIP and DINO to 3D point clouds, and then learning representations on top with SSL, which results in features that take context of the whole scene into account. We show that 3D-JEPA can be effectively fine-tuned for the localization task using a text-conditioned decoder head. The resulting model, LocateX, achieves state-of-the-art results in standard benchmarks like ScanRefer.

We present LocateX, a model for localizing objects in 3D scenes from textual referring expressions such as "chair near entryway door". It operates directly on sensor observation streams (RGB-D, camera pose, intrinsics), enabling practical deployment in robotics and AR devices. Key to LocateX is 3D-JEPA, a novel self-supervised learning algorithm applicable to sensor point clouds. It first projects features from 2D foundation models (CLIP, DINO, SAM) into 3D point clouds. Subsequently, it uses masked prediction in latent space as the SSL pretext task to learn contextualized point cloud features. LocateX finetunes an encoder pre-trained with 3D-JEPA along with a text-conditioned decoder head that jointly predicts 3D masks and bounding boxes. We find that LocateX achieves state-of-the-art results in standard referential grounding benchmarks, demonstrates robust generalization to novel environments, and even outperforms prior work that rely on privileged information like clean 3D meshes or instance segmentation.

==> sections/experiments_EOY.tex <==
\section{Experiments and Analysis - EOY 2024}
\label{sec:experiments}

\subsection{How does LAM3D compare to prior methods for 3D referential grounding benchmarks?}

\input{tables/main_table.tex}

First we compare the performance of our LAM3D model, described in Section~\ref{sec:methods}, against prior work. To do so, we consider three standard benchmarks for referential grounding -- SR3D, NR3D, and ScanRefer [cite]. We present the overall results in Table~\ref{table:main_table}. The original incarnation of these benchmarks provide access to ground truth bounding boxes of all the objects in the scene, and the task was to choose the correct one. Most prior methods operate under this setting. We instead chose to evaluate our model under realistic conditions, and assume access to only the underlying sensor stream, and do not rely on any annotations or human post-processing. Despite evaluating under this more stringent criteria, our model achieves SOTA results in these benchmarks, when compared with methods that require more explicit annotations. We additionally compare with more recent methods based on VLMs (e.g. VLM-grounder~\citep{xu2024vlmgrounder} and our reimplementation described in Appendix), and again find that LAM3D achieves superior results. We now discuss different components that lead to the performance gains of LAM3D.

\subsection{Understanding the impact of 3D-JEPA}

We first study the importance of 3D SSL for the results in LAM3D. In order to do so, we first device a series of experiments intended to tease apart various factors associated with 3D-JEPA and how it is used in the overall LAM3D model.

\input{tables/pretraining.tex}

\paragraph{\bf Is 3D SSL even necessary? Are lifted 2D foundation features sufficient?}
To answer these questions, we train the same localization head as used in LAM3D on the following point clouds: (a) RGB point cloud where no features beyond the color are used. This is intended to test if any features are necessary. (b) ConceptFusion~\citep{conceptfusion} which lifts 2D foundation features (specifically CLIP) to 3D. Each point in the point cloud contains color and object-level features. This can provide basic semantic understanding to the localization model, but scene-level understanding -- such as the placement of a chair relative to other objects in the scene -- must be learned along with the supervised localization task. (c) Finally, we also compare with ConceptFusion point clouds passed through a randomly initialized PTv3 encoder before the localization head. Both the localization head and PTv3 layers are finetuned in this experiment, which is in spirit same as (b) but with additional parameter counts in the PTv3 layer to be comparable to our final LAM3D model. We present the overall results in Table~\ref{table:pretraining_ablation}. We find overall that 3D-JEPA is crucial for localization. We also find that end-to-end finetuning of 3D-JEPA provides considerable benefits for the localization task.

% \paragraph{\bf What is the impact of masking patterns?} \todo{Move to appendix. Maybe for January.}

\paragraph{\bf On the choice of 2D foundation features} Input featurization matters: RGB-only, DINO-only, SAM-B + Clip-B < SAM-H + CLIP-L < SAM-H + Clip-L + DinoV2 

\input{tables/input_features}

\subsection{Analysis of Generalization}
\subsubsection{Zero-shot generalization to new datasets}
We collect new annotations to improve performance and study generalization. Details on our annotation task are available in \hyperref[sec:anno_appendix]{the appendix}. 

We find that our baseline model, trained only on existing benchmark data, achieves 48.5\% performance on a new held-out test set on ScanNet++. This is despite numerous domain shifts, which we decompose into the following axes:
\begin{enumerate}
\item \textbf{Linguistic:} A different annotator population and annotation task
\item \textbf{Scene:} A shift from full-room scans of small rooms to partial scans of much larger interiors\footnote{On ScanNet++, we "chunk" scenes into contiguous trajectories of 11 iPhone RGBD frames with a frameskip of 30 before annotation. This is a feature of our annotations, not of ScanNet, different capture setup, etc.}
\item \textbf{Object:} A shift in annotated object class distribution
\end{enumerate}
Additionally, we increase the generalization capabilities of our model by 

\subsubsection{Decomposing the domain gap}
For a more fine-grained analysis of the generalization capabilities of LAM3D, we devised a series of experiments to tease apart different axes of generalization. In particular, we aim to understand generalization to different linguistic queries and scenes. In order to do so, we create a new evaluation set on ScanNet++ and gradually ablate the training data to vary the gap between the train and eval domains. By doing so, we can precisely measure the change in performance due to each of these domain shifts.

\begin{enumerate}
    \item \textbf{$\Delta-$Linguistic } To measure the gap due to linguistic variance, we add training annotations collected on ScanNet using the same annotation instructions as on the evaluation set.
    \item \textbf{$\Delta-$Scenes } To measure the gap due to scene distribution and camera capture setup but \textit{not} query class distribution, we add training annotations on ScanNet++ which only cover instance classes available in ScanNet.
    \item \textbf{$\Delta-$Objects } To measure the gap due to query class distribution, we finally add in training annotations on ScanNet++ on object instances whose semantic class is not necessarily available in ScanNet.
\end{enumerate}

We find that there is a significant gap due to both the linguistic distribution and scene+object distribution, with around an X\% percent linguistic gap and a X\% percent scene+object gap. These gaps highlight the need for evaluation sets which are representative of downstream use-cases. They also suggest future research in increasing the robustness of the language encoder via additional training data, architectural adjustments, or LLM-powered data augmentation.

==> sections/experiments_disc.tex <==
\section{Experiments and Analysis}
\label{sec:experiments}

\begin{enumerate}
    \item \textbf{How does LAM3D compare to prior methods in 3D referrential grounding benchmarks?} We achieve SOTA. (\cref{table:main_table})
    \todo{[Discuss Q] Should we include VLM results?}

    \item \textbf{What is the impact of the pretraining recipe?}
    \begin{enumerate}
        \item pretraining is essential - compare from scratch (JEPA input goes directly into head without PTv3, frozen JEPA, finetuned JEPA - \cref{table:pretraining_ablation} \todo{[Discuss Q] Consider some other 3D backbone like ponder-v2 or PointContrast?}
        \item impact of masking patterns - random percent vs percent radius vs spatially consistent radius \todo{[Discuss] just linear probing or full fine-tuning? More of an appendix level detail. Mention conclusion in text form in the paper.}
        \item \textbf{Impact of 2D Foundation Features:} Input featurization matters: RGB-only, DINO-only, SAM-B + Clip-B < SAM-H + CLIP-L < SAM-H + Clip-L + DinoV2 
    \end{enumerate}

    \item \textbf{Generalization} - performance in out-of-domain settings (golden test set we collected and Fremont offline evals and robot experiments) - similar to \cref{table:main_table} but with only top baselines.
    - generalization to new queries/language (Ada's data) x generalization to new scan settings/devices (Fremont)
    
    \item \textbf{Localization Decoder ablations} \aravind{A good amount of these can go into appendix}
    \begin{enumerate}
        \item Transformer: (1) updating pointcloud features is necessary (2) order of cross-attentions is irrelevant (3) concatenating text features and learned queries works best.
        \item Task-Head: (1) MLP is necessary on the mask head (2) Explicitly attending to locations is necessary in bounding box head (3) Cosine similarity is not sufficient for the token predictions head. 
        \item Jointly predicting bboxes and masks. Why?
        \item Learned queries: (1) impact of increasing/decreasing the number of learned queries (2) the computational impact of non-parametric queries.
        \item Text encoder: Clip vs Roberta. Clip aligns better with pretrained features - how does this affect in-domain and o.o.d performance?
    \end{enumerate}

    \item \textbf{Scaling Model size} (decoder size) -- table with 4 model variants.  Perf vs param count on fixed data. Key insight: we expect larger models to help, and find this to hold in 3D as well?

    \item \textbf{Data Ablations} \todo{get clarity on this}

\end{enumerate}


\input{tables/main_table.tex}
\input{tables/pretraining.tex}

==> sections/intro.tex <==
%
\begin{figure}[b!]
    \centering
    \includegraphics[width=0.8\linewidth]{assets/teaser-fig-v001.png}
    \caption{\centering \todo{Teaser Figure}}
    \label{fig:teaser-figure}
\end{figure}
%
\section{Introduction}
\label{section:intro}
%
The world we inhabit is fundamentally 3D in nature. For AI systems to effectively assist us in day-to-day lives, whether through robots or smart glasses, they need an understanding of the 3D world grounded in human natural language. Consequently, the intersection of vision and language has seen an explosion of interest in recent years~\citep{Bordes2024VLMSurvey}. Tasks such as Visual Question Answering~\citep{schwenk2022aokvqa}, Embodied Question Answering~\citep{majumdar2023openeqa}, and object localization~\citep{gupta2019lvis} exemplify this trend. In this context, our work focuses on the task of 3D object localization via referring expressions~\citep{chen2020scanrefer}, which requires localizing an object in a 3D scene based on its textual description. Such descriptions can refer to the intrinsic attributes of the object (e.g., 'red chair') or its spatial relationship with other objects (e.g., 'chair closest to the entryway door').

Despite the importance, there is a scarcity of datasets that contain 3D object locations and their language descriptions. As a result, the task of 3D referential grounding remains largely unsolved. At one end of the spectrum are methods that train specialized models for this task~\citep{Jain2021BottomUT, chen2022vil3dref} on small benchmark datasets. They often require detailed 3D meshes and ground-truth proposals (e.g. instance segmentation of objects), which makes them difficult to scale up or deploy in real world settings on robots or smart glasses. At the other end of the spectrum are methods that try to leverage 2D VLMs for 3D tasks~\citep{xu2024vlmgrounder, zhu20233dvista}. While these methods can encode rich linguistic structures owing to their direct use of language models, they employ a simplistic and hand-crafted representation of the 3D world. As a result, these methods struggle to effectively encode the rich geometric information present in 3D scenes.

% new ver (WIP)
% To address these challenges, we propose a novel approach to 3D referential grounding, summarized in Figure~\ref{fig:teaser-figure}. Our key innovation is \textbf{3D-JEPA}, a novel self-supervised learning algorithm that leverages 2D foundation features to learn \textbf{contextualized 3D representations.}  
% and has two components. First, we have a pre-processing step and 3D representation backbone that converts RGBD sensor observation stream into a featurized point cloud representation. To realize and scale up this backbone, we developed \textbf{3D-JEPA}, a novel self-supervised learning algorithm applicable to sensor point clouds. To our knowledge, this is the first 3D representation backbone trained on scene-level point clouds. Furthermore, we emphasize that the 3D-JEPA training (and inference) is entirely self-supervised and does not require any ground-truth meshes or human post-processing. Secondly, we developed a novel \textbf{3D~localization~decoder} that operates on the 3D-JEPA point cloud and text queries to localize the desired object. Unlike prior mask decoder heads~\citep{Jain2021BottomUT, cheng2021mask2former}, our localization head attends to text tokens from the start, and uses interleaved cross-attention layers between the featurized points (from 3D-JEPA) and language tokens, which minimizes memory footprint and improves training stability. Through this combination, we achieve SOTA results on standard 3D referential grounding benchmarks, and demonstrate strong generalization to out-of-domain (OOD) scenes.

% old ver (placeholder)
To address these challenges, we propose a novel approach to 3D referential grounding. Our approach is summarized in Figure~\ref{fig:teaser-figure} and has two components. First, we have a pre-processing step and 3D representation backbone that converts RGBD sensor observation stream into a featurized point cloud representation. To realize and scale up this backbone, we developed \textbf{3D-JEPA}, a novel self-supervised learning algorithm applicable to sensor point clouds. To our knowledge, this is the first 3D representation backbone trained on scene-level point clouds. Furthermore, we emphasize that the 3D-JEPA training (and inference) is entirely self-supervised and does not require any ground-truth meshes or human post-processing. Secondly, we developed a novel \textbf{3D~localization~decoder} that operates on the 3D-JEPA point cloud and text queries to localize the desired object. Unlike prior mask decoder heads~\citep{Jain2021BottomUT, cheng2021mask2former}, our localization head attends to text tokens from the start, and uses interleaved cross-attention layers between the featurized points (from 3D-JEPA) and language tokens, which minimizes memory footprint and improves training stability. Through this combination, we achieve SOTA results on standard 3D referential grounding benchmarks, and demonstrate strong generalization to out-of-domain (OOD) scenes.

\aravind{Highlight two main components better: (a) SSL is especially important for 3D due to data scarcity and we leverage 2D foundation features in this pre-training to get better semantic understanding; (b) How to use the pre-trained backbone for grounding task without destroying the features.}

\subsection{Our Contributions} In summary, the key contributions of our work include:

\begin{enumerate}
    \itemsep0em
    \item \textbf{LAM3D -- SOTA results and strong OOD generalization.} Our primary contribution is the development of \textit{``Localize Anything Model in 3D''} (LAM3D) described in Figure~\ref{fig:teaser-figure}. LAM3D can operate directly on RGBD sensor streams and does not require any human annotations or post-processing. We find that on standard 3D referential grounding benchmarks (ScanRefer, SR3D, NR3D), LAM3D presents a significant advancement over the current best methods (\textbf{xx\%} $\rightarrow$ \textbf{yy\%}). 
    
    Crucially, LAM3D achieves these impressive results with fewer assumptions compared to prior models. Unlike prior work, LAM3D does not require ground truth region proposals, meshes, or surface normals, making it suitable for real-world deployment. When tested on a held-out multi-room apartment, we found that LAM3D could successfully localize objects different from the aforementioned benchmarks, and enable successful navigation and picking behaviors. The quality of results remained consistently strong across different sensing devices, underscoring the strong generalization and robustness qualities of LAM3D. We will open-source this model and hope that it will power a broad set of downstream applications. We describe the main components of our model below.
    
    \item \textbf{3D-JEPA -- A novel SSL method applicable to point clouds.} To encode the rich geometric and semantic structure of 3D scenes, we developed a new SSL method for point clouds, by extending the JEPA framework~\citep{Assran2023IJEPA, Bardes2024VJEPA}. 3D-JEPA is particularly well-suited for handling large point clouds where each point has a high feature dimension. In our instantiation, the point cloud feature dimension includes both native features (RGB) as well as 2D foundation features (CLIP, DINO) obtained from the underlying RGBD sensor stream. This allows our 3D backbone to understand the scenes at multiple layers of abstraction - from geometric/shape attributes, to object semantics, to scene layouts. We find 3D-JEPA to play a critical role in LAM3D performance - we see significant performance improvement compared to training a representation backbone from scratch, both in the benchmark tasks (\textbf{xx\%} $\rightarrow$ \textbf{yy\%}) as well as real-world evaluations (\textbf{xx\%} $\rightarrow$ \textbf{yy\%}). To our knowledge, 3D-JEPA is the first 3D representation backbone trained on large-scale point cloud datasets. We will open-source this model, and we hope its success inspires a field of SSL for 3D.

    \item \sergio{this should probably get folded into the LAM3D bullet rather than a separate point} \textbf{Novel text-conditioned 3D localization decoder.} Finally we also developed a new 3D localization decoder that operates on the 3D-JEPA features. This decoder is inspired by MaskFormer~\citep{cheng2021maskformer} and MDETR~\citep{} but leverages text tokens from the start. We use interleaved cross-attention layers between the points from 3D-JEPA and text/query tokens, resulting in minimal memory footprint despite the large size of the point clouds. The localization decoder has optimizes jointly 3D masking and bounding box heads. 

    % \item \todo{Gold standard annotated dataset. We need to discuss how to best tie it into the story. For now, it might be best to mention in the internal note, and include in paper downstream when we have trained models on it and have more numbers.}


\end{enumerate}


\iffalse
Despite the fact that we spend most of our time infront of a computer screen, the world is (un)fortunately 3D, and AI systems need to understand it to effectively assist us in day to day tasks..

\paragraph{Our Contributions} We developed a new algo, trained an awesome model, got SOTA results, and released it!
\fi

    % \item \textbf{SOTA model for RefExp from sensor point clouds} We developed a new model for 3D referential grounding on benchmarks like SR3D and NR3D. Furthermore, our model operates directly on sensor point clouds and does not require meshes or human annotations (both during training and inference), greatly enhancing its applicability. For example, we deploy our model on a robot in a previously unseen multi-room home, and show that it can successfully find and navigate to novel objects that were previously never seen during training. We achieve this model through two key innovations described below.
    % \item \textbf{Novel SSL method for 3D point clouds} We extend the JEPA framework previously used for images and videos to 3D sensor point clouds. \todo{Say more why JEPA is particularly well suited for this.} Can leverage 2D foundation features enabling rich generalization.
    % \item \textbf{Novel language-conditioned MaskDecoder architecutre} 
    % \item \textbf{New Dataset for 3D Referrential Grounding} \todo{Need to make it clear that we get SOTA even in the standard setup, as opposed to getting SOTA by training on more labeled data}

==> sections/methods.tex <==
\section{LAM3D: End-to-end model overview}
\label{sec:methods}
We start by providing a system overview, before diving into the details of our end-to-end approach.
%
\subsection{Overall System Architecture}
%
Figure~\ref{fig:teaser-figure} presents the overall system architecture of LAM3D. We operate in the simplified setting where we collect RGBD sensor observations in a static environment. This is true in most cases like homes where the scene is largely static in short intervals. LAM3D contains three modules: (1) computing featurized sensor point clouds from RGB-D sensor observations. (2) a point transformer v3 encoder which takes as input the featurized point cloud and outputs a latent featurized point cloud. This encoder is pre-trained via our novel pre-training algorithm named 3D-JEPA. Finally, (3) a language-conditioned 3D-localization head that operates on a featurized pointcloud to localize and ground the queried object. LAM3D does not require any human annotation at inference time and operates directly on sensor streams. We'll start by describing the featurization of our point clouds.

% [Franzi] don't understand the purpose of this section here - commenting it out. Maybe something for related work/intro?
%\textbf{Why 3D point clouds?} When operating with sensor streams, we can either chose a video-first approach that directly operates on frames, or leverage a 3D representation of the sensor stream. In this work, we chose the latter. This is motivated by the desire to operate on long horizon sensor streams and the hypothesis that a 3D representation can enable better spatial understanding of the scene. A common data format for 3D is point cloud – a set of points with location and color attributes, which can be interpreted as samples from visible surfaces in the scene. Point clouds are easy to construct from sensors, faithfully reflect the geometry of the scene, and avoid quantization artifacts that can arise from a regular 3D grid structure. These advantages combined with advances in deep learning architectures capable of processing point clouds~\citep{iek20163DUnet, Engel2020PointTransformer, Wu2023PointTransformerV3} motivate our choice for the 3D format.

\subsection{Computing featurized point clouds utilizing SAM, CLIP and DINO}
%
Given an RGBD observation stream from a camera (along with pose and intrinsics), standard SLAM systems provide a way of constructing RGB point clouds. In addition to just color, we would like to add additional 2D foundation features (e.g. from CLIP, DINO) to the points to aid with better semantic understanding. To do so, we process each image in the observation stream with SAM~\citep{kirillov2023segment} to get segmentation masks and encode each segmented mask with CLIP to get object level features. \franzi{we're missing a description on how DINO features are computed. Please add. + describe what happens with "holes" - points that didn't fall within a SAM mask - I believe they just have the RGB feature} These features are then aggregated over frames~\citep{conceptfusion} and added to the point features. This process results in a featurized point cloud $\mathbf{FPtC} = \{ (x_i, y_i, z_i, \mathbf{f}_i ) \}_{i=1}^N $ where $\mathbf{f}_i \in \mathbb{R}^d$ is the feature vector of the $i^{th}$ point. In our implementation, $\mathbf{f}_i$ combines RGB, CLIP, and DINO features, but in principle can leverage any 2D feature backbone. $\mathbf{FPtC}$ can then be passed either through an language-conditioned mask or bbox decoder directly, or can first be passed through an encoder that further processes the features. In this work we evaluate both possibilities and find that when further processing featurized pointclouds through a 3D-JEPA pre-trained backbone we achieve better performance. 

\subsection{Self-supervised pre-training of an encoder via 3D JEPA}
%
\aravind{Some more motivations we want to highlight: (1) Pre-training is particularly useful for 3D since labelled data is more scarce. Also motivates leveraging 2D foundation features. (2) Lifting 2D to 3D directly (i.e. the ``raw feature'' point cloud input to JEPA) is insufficient since features are per-point and scene-level context is absent - decoder has to do a LOT of work - show with experiments. }

% \begin{itemize}
%     \item While JEPA SSL methods have been shown to learn good features on raw inputs, 3d data is limited so bootstrap with 2d foundational features. Experiment: compare rgb, dino, clip, dino + clip input to jepa representations
%     \item Cannot solely use 2d foundational features. For example, dino representation can predict depth. Having the depth from a particular camera view is meaningless when its a point in a pointcloud. Also, clip does not capture global information and is noisy and sometimes meaningless (mask of blank wall). Experiments: just 2d foundation representations to decoder
%     \item SSL can extract the predictable information from 2d foundational models and fuse the knowledge of clip and dino into one representation. Same experiments as above
% \end{itemize}

\begin{figure}[b!]
    \centering
    \includegraphics[width=0.8\linewidth]{assets/JEPA alg illustration.png}
    \caption{\centering Overview of the 3D-JEPA training framework.}
    \label{fig:enter-label}
\end{figure}

Our models encoder takes as input the featurized pointcloud $\mathbf{FPtC}$ from above, and predicts latent feature pointcloud $\mathbf{LPtC}$. This encoder is pre-trained via 3D-JEPA, a novel self-supervised pre-training algorithm inspired by JEPA~\citep{Assran2023IJEPA, Bardes2024VJEPA}.

\franzi{it's not like MAE can't be applied to 3d pointclouds (there is prior work doing so - for instance PointMAE) - so we should reframe this next paragraph a bit. Also might fit better into the related work section}
Masked prediction has emerged as a dominant paradigm for SSL, demonstrating success in both NLP~\citep{Devlin2019BERT} and vision~\citep{He2021MAE}. However, the lack of a regular grid structure for point clouds poses a challenge to directly extend this approach. Point clouds are order invariant and can have variable number of points, which makes this a set-value to set-value prediction problem. This rules out standard losses like MSE and cross-entropy. Secondly, losses applicable to set values like Chamfer or Hausdorff distance take only the location of predicted points into account. Consequently, the learned representations may not meaningfully use the feature vectors associated with points. Instead, we take inspiration from JEPA~\citep{Assran2023IJEPA, Bardes2024VJEPA} and propose an encoder-predictor framework that performs masked prediction in a learned latent space. This results in an SSL framework that can simultaneously capture various aspects of a 3D scene such as shapes, semantics, and overall spatial layout.

Concretely, let $\mathbf{PtC}$ be a point cloud with ``base features''. 3D-JEPA trains two transformer models $E_\theta(\cdot)$ and $P_\phi(\cdot)$ using the following objective,
\begin{equation}
    \min_{\theta, \phi} \ \  \Big|\Big| P_\phi \left( E_\theta(\mathbf{\tilde{PtC}}), M \right) - \mathrm{sg}\left( \bar{E}_\theta (\mathbf{PtC}) \right) \Big|\Big|,
\end{equation}
where $\tilde{\mathbf{Ptc}}$ denotes a masked view of the point cloud, $M$ is a mask variable describing regions that were masked, and $\mathrm{sg}(\cdot)$ is the stop-grad operator. Finally, $\bar{E}_\theta(\cdot)$ is the exponentiated moving average version of the encoder, which is important to prevent the representation from collapsing. \aravind{Need to explain how we aggregate losses across points and mini-batch.}

\paragraph{\bf Model Architectures} Unlike images or voxels that contain a regular grid structure, point clouds are order invariant and set-valued. U-Net~\citep{iek20163DUnet}, PointNet~\citep{Qi2016PointNetDL} DeepSets~\citep{Zaheer2017DeepSets} and PointTransformer~\citep{Engel2020PointTransformer} have all emerged as promising architectures for point clouds. For our implementation of 3D-JEPA, we use PointTransformer-v3~\citep{Wu2023PointTransformerV3} for encoder and a transformer with sparse attention for the predictor, which we found beneficial owing to the large size of our point-clouds. \todo{Should we talk about chunking here?}  \aravind{Section under construction}

\paragraph{\bf Masking Patterns} We found the choice of masking pattern to play a crucial role in the quality of representations learned, consistent with prior literature in JEPA~\citep{Assran2023IJEPA, Bardes2024VJEPA}. Figure~\ref{fig:masking_patterns} \aravind{Section under construction}

\subsection{Language-conditioned 3D Mask and BBox-Decoder}
The 3D mask decoder takes as input a featurized point cloud representation from 3D-JEPA and a language query, and outputs a set of instance masks, bounding boxes, and text-to-prediction correspondence scores. The architecture consists (1) a transformer decoder that fuses point cloud and language features, (2) parallel prediction heads for masks and bounding boxes, and (3) a token-prediction head that grounds predictions to noun phrases in the input text. We explain
the various components of this decoder below.
\franzi{please add a summary statement of what is novel, also add a citation for the closest model out there}

\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{assets/3d_mask_decoder.pdf}
    \caption{\centering Our 3D Mask Decoder}
    \label{fig:3d_mask_decoder}
\end{figure}

\textbf{Feature Processing:} Point cloud features from 3D-JEPA are first projected to the model's working dimension through a linear layer followed by normalization. Similarly, we encode the input text using a CLIP (CITE) text encoder and project the resulting token features. We also maintain a set of learned object queries that are trained end-to-end with the model (similar to DETR, Maskformer, ...)

\textbf{Transformer:} The core of our decoder is a stack of transformer layers that iteratively refine object queries by attending to both point cloud and language features. Each layer consists of three attention modules operating in sequence (see \cref{fig:3d_transformer}):

\begin{itemize}
    \item \textbf{Query self attention:} The concatenated query and text features attend to themselves, enabling information exchange between different queries and allowing them to specialize in different objects
    \item \textbf{Query to pointcloud cross-attention:} Queries attend to point cloud features gathering instance-relevant spatial information
    \item \textbf{Pointcloud to query cross-attention:} Point cloud features are updated by attending to the refined queries
\end{itemize}

Consistent with observations in RODIN [cite] \sergio{The transformer above is from RODIN so we shouldn't claim it as novel}, we find that updating point cloud features through cross-attention is crucial for mask prediction performance. This bidirectional information flow allows the model to better understand the relationships between language descriptions and spatial regions in the point cloud.

\textbf{Prediction Heads:} The refined features from each transformer layer are passed through three parallel prediction heads:
\begin{enumerate}
    \item \textbf{Mask Head:} Computes dot products between query features and point cloud features to predict per-point segmentation masks.
    \item \textbf{Bounding Box head:} Processes query features through a transformer to regress the 3D bounding box parameters (center and dimensions)
    \item \textbf{Token Prediction Head:} Produces scores relating each query (associated to a mask and bbox given previus heads) to noun phrases in the input text, enabling explicit grounding of predictions to language.
\end{enumerate}

During training, we apply deep supervision (the loss is computed to outputs from all decoder layers for faster convergence) similar to DETR [cite]; the final predictions are taken from the last layer during inference. The mask predictions are supervised using binary cross-entropy loss and dice loss on ground truth instance masks (akin to maskformer), while the bounding box head uses a combination of L1 loss on box parameters and generalized IoU loss. The token prediction head is trained using a focal loss for query-to-prediction alignment. During training, we follow DETR (cite) to apply Hungarian Matching between queries and ground-truth objects. For details see Appendix.

\subsection{LAM3D Model Card}
We opensource a model trained with the aforementioned components, and we evaluate its performance in Section~\ref{sec:experiments}. We opensource two components (1) The pre-trained Jepa PTV3 encoder and (2) LAM3D with the Jepa PTV3 encoder fine-tuned for the referring expresion task + localization decoder.


\textbf{3D-JEPA backbone} The backbone is trained on ScanNet and ARKit [cite]. For pre-processing, we used SAM-H and CLIP-L + DINO-v2 [cites] for 2D foundation features. The encoder is a \textbf{xx million} parameter PointTransformer-v3 [cite] model with a feature dimension of $128$. The predictor is a \textbf{yy million} parameter transformer with sparse attention pattern. We train the model with the serialized percent masking pattern depicted in Figure~\ref{fig:masking_patterns}. 

\textbf{LAM3D:} We train our localization decoder from scratch and fine-tune the 3D-JEPA pretrained backbone. Our model is trained jointly across several referring expression benchmarks. Specifically, we train and evaluate on the 3D referential grounding datasets of SR3D, NR3D \cite{Achlioptas2020ReferIt3DNL} and ScanRefer \cite{chen2020scanrefer}. \ada{We also collect and train using an additional 75,000 annotations across ScanNet-v2 and ScanNet++-v1. (but these are not in our current best yet)} LAM3D has \textbf{xx million} parameters. 

\todo{Low-level training and pretraining details (lr, optimizers, schedulers, ...) -- send to appendix?}



==> sections/related-work.tex <==
\section{Related Work}
\label{sec:related_work}

\paragraph{\bf Self Supervised Learning (SSL)} and more broadly representation learning for 3D data like point clouds is relatively under-explored compared to 2D vision~\citep{Fei2023SSL3DSurvey}. Among the few explorations, most have focused on learning representations for individual objects using object-level point clouds~~\citep{Sauder2019SelfSupervisedDL, Pang2022PointMAE, Zhang2022PointM2AE}. PointMAE~\citep{Pang2022PointMAE, Zhang2022PointM2AE} and PointBERT~\citep{Yu2021PointBERT} use masked modeling techniques for object-level point clouds and show that the resulting representations can be effective for tasks like classification and segmentation. They differ crucially from our work on two fronts. Firstly, our work focused on scene-level point clouds which contain significantly more points and objects compared to single object point clouds used in prior work. Secondly, we operate on point clouds with high feature dimensions, as opposed to RGB point clouds in prior work. In our experiments we found that a naive instantiation of masked modeling is ineffective due to a combination of these factors. PointCLIP~\citep{Zhang2021PointCLIP} leverages 2D foundation features for CLIP, but again has been studied only for object-level point clouds. Prior works have also explored contrastive learning methods for point cloud data~\citep{Xie2020PointContrast, Zhang2021DepthContrast}, which encourages invariant representations to different types of transformations. Ponder-v2~\citep{zhu2023ponderv2} proposes an SSL pretext task based on differentiable rendering into 2D. We refer readers to a recent survey on SSL for point clouds for additional references~\citep{Fei2023SSL3DSurvey}.


% has led to tremendous advances in recent years, in both computer vision and NLP. However, SSL for 3D vision is still not mature, with most works still training from scratch on target datasets~\citep{Hou2020ExploringD3}. Among the few explorations in SSL for 3D, most have focused on learning representations for individual objects~\citep{Sauder2019SelfSupervisedDL, Pang2022PointMAE, Zhang2022PointM2AE}, with some explorations into scene-level point clouds~\citep{zhu2023ponderv2} \todo{cite more}. However, to our knowledge, no prior work has focused on point clouds with high feature dimensions beyond color and intensities. In contrast, our 3D-JEPA backbone is trained using both native point cloud features as well as 2D foundation features. In principle, this combination of features can allow a representation backbone to understand the scene at various levels of abstractions like geometry/shape, object semantics, and scene layouts. We note that several prior methods, especially those based on masked auto-encoding, cannot be extended to high point feature dimensions, due to their reliance on losses that are specific to point coordinates. We hope that our strong results with 3D-JEPA inspire more work on 3D SSL.

% \franzi{Let's checkout this survey paper on self-supervised pre-training on pointclouds for additional work: Self-supervised Learning for Pre-Training 3D
% Point Clouds: A Survey}

\paragraph{\bf 3D Referential Grounding} Recent years have seen renewed interest in tasks at the intersection of perception and language, such as visual grounding~\citep{zhang2023recognize, liu2023grounding, ren2024groundedSAM} and visual question answering~\citep{agrawal2016vqa, sermanet2023robovqa, majumdar2023openeqa}. Of particular relevance to this work are 3D referrential grounding benchmarks, such as SR3D, NR3D, and ScanRefer~\citep{Achlioptas2020ReferIt3DNL}, which require localizing objects mentioned in a language utterance using observations of a 3D scene. We note that the original instantiations of these benchmarks provide access to ground-truth bounding boxes of all objects in the scenes as input (including at test time), and the task is to simply select the correct bounding box. In contrast, we wish to develop methods that can operate directly on sensor observation, without requiring any annotations. Few prior works have operated under this setting.

Current approaches for 3D grounding fall under two classes of methods. First are end-to-end models designed explicitly for this task, that either directly predict the bounding box~\citep{Luo20223DSPS, Jain2021BottomUT}, or provide probabilities for region proposals~\citep{chen2022vil3dref, zhu20233dvista, zhu2024PQ3D}. The former approaches have so far not been demonstrated on sensor point clouds or scaled up to multiple datasets. The latter approaches require an external region proposal mechanism, which is often difficult in 3D, and are prone to any failures there. The second class of methods aim to leverage 2D foundation models (VLMs) for 3D tasks, either by finetuning heads for 3D localization~\citep{hong20233dllm} or through use of tools~\citep{Yang2023LLMGrounderO3, xu2024vlmgrounder}. While these methods inherit the strong generalization capabilities of foundation models, they rely on tools for grounding and inherit their weaknesses. In the broader context, one could interpret LocateX as a powerful tool that such agents can leverage to perform better in the future. 


% \todo{Talk about JEPA, DINO, CLIP}. However, advances in 3D SSL has been comparitively lacking. Focus is primarily on object-level point clouds as opposed to full scenes. Talk about PTv3 and Saining's papers.  


==> sections_EOY/abstract.tex <==
todo

==> sections_EOY/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this work, we introduced LocateX, a model for localizing objects in 3D from textual referring expressions. Our approach leverages 3D-JEPA, a novel self-supervised learning method for point clouds. It first projects features from 2D foundation models (like SAM, CLIP, DINO) into 3D point clouds. Subsequently, it performs SSL on top of these lifted features with a pretext task of masked prediction in latent space - i.e. predict latent features of masked regions using the remainder of the scene. We showed that this enables the learning of contextualized representations -- i.e. features of a particular point take into account the whole scene. We also showed that a backbone pre-trained with 3D-JEPA can be effectively finetuned for the task of RefExp, using a mask-and-box decoder, that ultimately results in LocateX. We show that LocateX achieves state-of-the-art results in standard RefExp benchmarks. Furthermore, unlike prior work, LocateX only requires sensor point clouds which are easy to construct using existing SLAM systems, making it suitable for applications like robotics and smart glasses.

==> sections_EOY/experiments_EOY.tex <==
\section{Experiments and Analysis}
\label{sec:experiments}

\subsection{How does LocateX compare to prior methods for 3D referential grounding benchmarks?}

\input{tables/main_table.tex}

First we compare the performance of our LocateX model, described in Section~\ref{sec:methods}, against prior work. To do so, we consider three standard benchmarks for referential grounding -- SR3D, NR3D, and ScanRefer [cite]. We present the overall results in Table~\ref{table:main_table}. The original incarnation of these benchmarks provide access to ground truth bounding boxes of all the objects in the scene, and the task was to choose the correct one. Most prior methods operate under this setting. We instead chose to evaluate our model under realistic conditions, and assume access to only the underlying sensor stream, and do not rely on any annotations or human post-processing. Despite evaluating under this more stringent criteria, our model achieves SOTA results in these benchmarks, when compared with methods that require more explicit annotations. 
%We additionally compare with more recent methods based on VLMs (e.g. VLM-grounder~\citep{xu2024vlmgrounder} and our reimplementation described in Appendix), and again find that LocateX achieves superior results. 
We now discuss different components that lead to the performance gains of LocateX.

\subsection{Understanding the impact of 3D-JEPA}

We first study the importance of 3D SSL for the results in LocateX. In order to do so, we first device a series of experiments intended to tease apart various factors associated with 3D-JEPA and how it is used in the overall LocateX model.

\input{tables/pretraining.tex}

\paragraph{\bf Is 3D SSL even necessary? Are lifted 2D foundation features sufficient?}
To answer these questions, we train the same localization head as used in LocateX on the following point clouds: 
%(a) RGB point cloud where no features beyond the color are used. This is intended to test if any features are necessary. \aravind{commenting this out since we don't yet have this table entry. Expect to be bad. Run later.}
(a) Lifted 2D foundation features, following the ConceptFusion~\citep{conceptfusion} framework. We lift both CLIP and DINO features for fair comparison on leveraging the same 2D foundation models. (b) We also compare with the same lifted features, but first passed through a randomly initialized PTv3 encoder before the localization head. Both the localization head and PTv3 layers are finetuned in this experiment for a fair comparison with 3D-JEPA in terms of parameter count. We present the overall results in Table~\ref{table:pretraining_ablation}. We find overall that 3D-JEPA outperforms both variants of using lifted 2D features. Additionally, while frozen 3D JEPA features already outperform the use of lifted 2D features, we observe that finetuning the backbone for 3D-RefExp provides considerable gains. Notably, these gains are absent when simply using 2D foundation features.

\paragraph{\bf Does 3D JEPA learn contextualized representations?} The key premise of SSL on the lifted features is the ability for points to attend to different regions of the scene and learn representations that are contextualized. To test if this indeed is the case, we devise a point-wise probing experiment for localization. We train a probe that operates on a text description (e.g. "chair near entryway door") and features of a single point to classify if the point satisfies the description or not. To be successful in this, the point features must capture details about the object contextualized in the scene, since the probe cannot attend to the whole scene. We find that 3D-JEPA a point-probe success of 43\% in contrast to 33\% for ConceptFusion (lifted 2D features), confirming that it indeed learns representations that are more contextualized.

\paragraph{\bf On benefiting from advances in 2D foundation features} Due to the massive amount of data available on the internet, 2D foundation models have been consistently improving. Do those advances also improve results in 3D? If so, this provides a powerful opportunity to leverage progress and advances there. To tease this apart, we trained variants of the LocateX model using different 2D foundation features. This goes through the full development process of lifting 2D features, pre-training the 3D backbone using said features, and end-to-end finetuning for 3D-RefExp using the localization heads. The results are presented in Table~\ref{}. We find that using larger models (CLIP-L, SAM-H) improves results over the smaller variants (CLIP-B, MobileSAM) suggesting benefits from scaling laws. Additionally, the use of both CLIP and DINO improves results considerably over using CLIP alone. Thus, we find promising evidence that improvements in 2D foundation models do indeed translate to 3D. 
% \daniel{Curious reader may wonder what the performance is with just XYZRGB features. I remember these numbers were discussed back then. Worth mentioning if space allows? [aravind] Yes, but we don't have the numbers right now. We should include for ICML.}


% \daniel{No decoder arch / ablation experiments? I'd expect either section 2.4 or experiments to contain some explicit answers to the question "why choose this decoder architecture?".}\franzi{agreed}

\input{tables/input_features}

\subsection{Out-of-Domain Generalization}

\paragraph{\bf Zero-shot generalization to new datasets} We collected new annotations to study if LocateX overfits to the specific details/peculiarities of the benchmark. Details on our annotation task are available in \hyperref[sec:anno_appendix]{the appendix}. We find that LocateX trained only on the standard benchmark training splits achieves 48.5\% performance on a new held-out test set on ScanNet++. This is despite numerous domain shifts like: (1)~\textbf{Linguistic:} A different annotator population and annotation task. (2)~\textbf{Scene:} A shift from full-room scans of small rooms to partial scans of much larger interiors. (3)~\textbf{Object:} A shift in annotated object class distribution.
% \begin{enumerate}
% \item \textbf{Linguistic:} A different annotator population and annotation task
% \item \textbf{Scene:} A shift from full-room scans of small rooms to partial scans of much larger interiors\footnote{On ScanNet++, we "chunk" scenes into contiguous trajectories of 11 iPhone RGBD frames with a frameskip of 30 before annotation. This is a feature of our annotations, not of ScanNet, different capture setup, etc.}
% \item \textbf{Object:} A shift in annotated object class distribution
% \end{enumerate}
Overall, this suggests that our model is quite robust. Additionally, we will release the new annotations we collected, for use in potential future benchmarks for 3D-RefExp. /todo{Are we allowed to say this?}

\paragraph{\bf Deployment on Robot} As outlined earlier, our model is capable of working with sensor streams and does not require human intervention at test time (e.g. for mesh refinement or instance segmentation). We deployed our LocateX model on a Spot robot in a held out apartment scene. This differs considerably from our training conditions like: (1) multi-room test apartment vs single-room training scenes; (2) sensor stream for robot camera vs from iPhone during training; (3) different objects and queries specialized to the test scene (e.g. "plushy toy"). We made the robot tour the apartment to build up the 3D representation, and then tasked the robot with locating an object of interest, navigating to it, and picking it up. We found success in 7/10 trials, with baselines achieving a max success rate of 3/10. We note that navigation and pick-up uses pre-trained skills, and localization uses our model. Additional details are provided in the appendix.

% =====
\iffalse
\subsubsection{Decomposing the domain gap}
\aravind{Ada, can we remove this for EOY and add back in Jan. I think it's a bit hard to make definitive statements here with the current set of experiments.}
For a more fine-grained analysis of the generalization capabilities of LocateX, we devised a series of experiments to tease apart different axes of generalization. In particular, we aim to understand generalization to different linguistic queries and scenes. In order to do so, we create a new evaluation set on ScanNet++ and gradually ablate the training data to vary the gap between the train and eval domains. By doing so, we can precisely measure the change in performance due to each of these domain shifts.

\begin{enumerate}
    \item \textbf{$\Delta-$Linguistic } To measure the gap due to linguistic variance, we add training annotations collected on ScanNet using the same annotation instructions as on the evaluation set.
    \item \textbf{$\Delta-$Scenes } To measure the gap due to scene distribution and camera capture setup but \textit{not} query class distribution, we add training annotations on ScanNet++ which only cover instance classes available in ScanNet.
    \item \textbf{$\Delta-$Objects } To measure the gap due to query class distribution, we finally add in training annotations on ScanNet++ on object instances whose semantic class is not necessarily available in ScanNet.
\end{enumerate}

We find that there is a significant gap due to both the linguistic distribution and scene+object distribution, with around an 8 percent linguistic gap and a 12.5 percent scene+object gap. These gaps highlight the need for evaluation sets which are representative of downstream use-cases. They also suggest future research in increasing the robustness of the language encoder via additional training data, architectural adjustments, or LLM-powered data augmentation.

\todo{update results and interpretation on newer model}


\begin{tabular}{l|ccccccc}
Eval Set: & SR3D & NR3D & ScanRefer & SN & SN++ & ARKit & FRE \\
\hline
Training Set: \\
\hline
1. SR3D+NR3D+ScanRefer & 58.2 & 44.0 & 50.0 & 44.9 & 48.5 & - & 13.0 \\
2. 1 + New annos (ScanNet) & 60.0 & 45.7 & 52.4 & \textbf{52.7} & \textbf{56.5} & + & \textbf{28.7} \\
3. 2 + New annos ScanNet++ (SN classes only) & - & - & - & - & + & + & + \\
4. 2 + New annos ScanNet++ (all SN++ classes) & 60.0 & 46.5 & 54.0 & 54.5 & \textbf{69.0} & + & \textbf{35.6} \\
\end{tabular}



\fi

==> sections_EOY/intro.tex <==
\section{Introduction}
\label{section:intro}

%
\begin{figure}[b!]
    \centering
    \includegraphics[width=\linewidth]{assets/teaser-fig-v004.png}
    \caption{\textbf{System Architecture of LocateX}, which operates in three phases. In \textbf{Phase1: preprocessing}, the system constructs a point cloud with ``lifted'' features from 2D foundation models that provide local information. In \textbf{Phase2: Contextualized Representation} these lifted features are passed through the pre-trained 3D-JEPA encoder which allows points to attend to each other, providing a contextualized representation for the whole scene. Finally, in \textbf{Phase3: 3D Localization}, a 3D decoder head uses the text query and 3D representation from JEPA encoder to localize the referred object. 
    % \todo{Improve figure quality, change phase names to reflect caption -- remove "maskformer"}
    }
    \label{fig:teaser-figure}
\end{figure}
%
 
The world we inhabit is fundamentally 3D in nature. For AI systems to effectively assist us in day-to-day lives, say through robots or smart glasses, they need an understanding of the 3D world grounded in human natural language. As a step towards this goal, we study the task of 3D localization via referring expressions~\citep{chen2020scanrefer}, or simply 3D-RefExp, which sits at the intersection of 3D vision and language. Concretely, the task is to localize an object in a 3D scene based on its textual description that can range from intrinsic attributes (e.g. "red chair") to spatial relationships (e.g. "chair closest to the entryway door"). In this work, we develop LocateX, a system that achieves SOTA results in benchmarks for 3D localization. The key innovation powering LocateX is 3D-JEPA, a novel self-supervised learning (SSL) algorithm that can use 2D foundation features to learn contextualized 3D representations. 

The task of 3D localization from referring expressions is challenging to date. At one end of the spectrum are methods that train specialized models for this task~\citep{Jain2021BottomUT, chen2022vil3dref} on small benchmark datasets. They often require human annotation, in the form of detailed 3D meshes or object instance segmentation, making them difficult to deploy in real-world devices. At the other end of the spectrum are methods that try to leverage 2D VLMs for 3D tasks~\citep{xu2024vlmgrounder, zhu20233dvista}. While these methods can encode rich linguistic structures owing to their direct use of language models, they employ a simplistic and hand-crafted representation of the 3D world. % As a result, these methods struggle to effectively encode the rich geometric information present in 3D scenes. In contrast to these works, we seek a method that can understand 3D scenes at various levels, and can ultimately work with sensors onboard robots and smart glasses.


Our system, LocateX, is described in Figure~\ref{fig:teaser-figure} and has three phases. We first leverage the underlying sensor observation stream (RGBD, camera pose, and intrinsics) to lift features from 2D foundation models to 3D point clouds, which is similar to prior work like ConceptFusion~\citep{conceptfusion}. Subsequently we leverage a transformer model to transform these ``lifted'' features into learned 3D-JEPA features that are contextualized for the scene. Concretely, the lifted foundation features help with local understanding (e.g. an object is a ``chair''), while the learned 3D-JEPA features provide contextual understanding taking the whole scene into account (e.g. chair close to the door, in the bedroom etc.). This backbone is initially pre-trained with SSL, and subsequently finetuned for the 3D-RefExp task. In the final phase, we use a 3D localization head inspired by Mask2Former~\citep{cheng2021mask2former} that uses interleaved cross-attention layers between the 3D-JEPA features and text query to localize the object of interest. This system overall operates on sensor streams from devices like robots and smart glasses without requiring any human intervention, like 3D mesh refinement or instance segmentation.

\textbf{Our Contributions} To summarize, the main contributions of this work are three-fold and outlined below.

\begin{enumerate}

    \item \textbf{3D-JEPA} -- A novel SSL method that can learn contextualized representations of 3D scenes. It proceeds by first lifting features from 2D foundation models to 3D point clouds, which provides local understanding, such as an object is a "chair". Subsequently, we setup an SSL pretext task in an encoder-predictor framework that requires predicting latent embeddings of randomly masked regions in the point cloud. We show that the resulting 3D-JEPA features are contextualized for the scene. While the features lifted from 2D foundation models provide local understanding (e.g. object is a ``chair''), the learned 3D-JEPA features encode information taking the whole context of the scene into account (e.g. chair is close to the door, in the bedroom). Loosely, this is analogous to word embeddings~\citep{Mikolov2013word2vec} vs contextualized embeddings~\citep{Devlin2019BERT} in NLP.

    \item \textbf{LocateX} - a model for 3D RefExp (see Figure~\ref{fig:teaser-figure}) that achieves SOTA benchmark results and strong out-of-domain generalization. It builds on the pre-trained 3D-JEPA backbone and finetunes it for the 3D RefExp task using a localization head that performs interleaving cross-attention between the 3D features and text queries, and employs a joint mask-box prediction strategy to handle sensor noise. On standard 3D RefExp benchmarks (ScanRefer, SR3D, NR3D), LocateX achieves SOTA results compared to prior work (\textbf{58.8\%} $\rightarrow$ \textbf{61.2\%}). Crucially, LocateX achieves these impressive results with fewer assumptions compared to prior models. LocateX does not require ground truth region proposals, meshes, or surface normals, making it suitable for real-world deployment. When comparing to prior work under similar assumptions~\citep{Jain2021BottomUT}, LocateX presents a significant advancement (\textbf{40.7\%} $\rightarrow$ \textbf{61.2\%}). Testing on a held-out and multi-room apartment in the real-world, we found that LocateX could successfully localize objects different from aforementioned benchmarks, and enable successful navigation and picking behaviors.

    \item \ada{\textbf{LX3D} - A new dataset for 3D RefExp which spans ScanNet, ScanNet++, ARKitScenes, and a held-out apartment used for robot trials\todo{section link to robot trials}. This new data improves the performance of our model by around 3 percent on existing in-domain benchmarks and around 12 percent on new held-out evaluations. It also allows us to study a localization model's ability to generalize to new capture setups and independent samplings of indoor environments.}
\end{enumerate}

==> sections_EOY/methods.tex <==
\section{LocateX: System Overview and Training}
\label{sec:methods}
We start by providing a system overview, before diving into the details of our approach.
%
\subsection{Overall System Architecture}
%
Figure~\ref{fig:teaser-figure} presents the overall system architecture of LocateX. We operate in the simplified setting where we collect RGBD sensor observations in a static environment. This is true in most cases like homes where the scene is largely static in short intervals. LocateX contains three modules: (1) Point cloud with ``lifted'' features: pre-processing the sensor stream to construct input point cloud that lifts 2D foundation features to 3D. (2) Learned 3D-backbone for contextualized features: A PointTransformer-v3~\citep{Wu2023PointTransformerV3} encoder which operates on lifted features and learns a contextualized 3D representation. This encoder is pre-trained with 3D-JEPA, our novel SSL algorithm. Finally, (3) finetuning for 3D-RefExp using a text-conditioned 3D-localization head that operates on the learned features to localize the query object. LocateX does not require any human annotation at inference time and operates directly on sensor streams. 

\subsection{Pre-Processing: Lifting 2D Foundation Features to 3D Point Clouds}
%
Given an RGBD observation stream from a camera (along with pose and intrinsics), standard SLAM systems provide a way of constructing RGB point clouds. In addition to just color, we would like to add additional 2D foundation features (e.g. from CLIP, DINO) to the points to aid with better semantic understanding. To do so, we process each image in the observation stream with SAM~\citep{kirillov2023segment} to get segmentation masks and encode each segmented mask with CLIP to get object level features. Additionally, we leverage DINO-v2 to get patch level features for each image. Each point is assigned features based on which mask/patch they belong to, and then aggregated over frames~\citep{conceptfusion}. This process results in a featurized point cloud $\mathbf{PtC}_{\textrm{lift}} = \{ (x_i, y_i, z_i, \mathbf{f}_i ) \}_{i=1}^N $ where $\mathbf{f}_i \in \mathbb{R}^d$ is the feature vector of the $i^{th}$ point. In our implementation, $\mathbf{f}_i$ combines RGB, CLIP, and DINO features, but in principle can leverage any 2D feature backbone. $\mathbf{PtC}_{\textrm{lift}}$ can then be passed either to a 3D localization head directly, or can first be passed through an encoder that further processes the features. In this work we evaluate both possibilities and find that using an additional encoder pre-trained with 3D-JEPA leads to substantially better results. 

\subsection{3D-JEPA: Learning Contextualized Representations with SSL}
%
% \aravind{Some more motivations we want to highlight: (1) Pre-training is particularly useful for 3D since labelled data is more scarce. Also motivates leveraging 2D foundation features. (2) Lifting 2D to 3D directly (i.e. the ``raw feature'' point cloud input to JEPA) is insufficient since features are per-point and scene-level context is absent - decoder has to do a LOT of work - show with experiments. }

% \begin{itemize}
%     \item While JEPA SSL methods have been shown to learn good features on raw inputs, 3d data is limited so bootstrap with 2d foundational features. Experiment: compare rgb, dino, clip, dino + clip input to jepa representations
%     \item Cannot solely use 2d foundational features. For example, dino representation can predict depth. Having the depth from a particular camera view is meaningless when its a point in a pointcloud. Also, clip does not capture global information and is noisy and sometimes meaningless (mask of blank wall). Experiments: just 2d foundation representations to decoder
%     \item SSL can extract the predictable information from 2d foundational models and fuse the knowledge of clip and dino into one representation. Same experiments as above
% \end{itemize}



Our model takes as input the lifted features $\mathbf{PtC}_{\textrm{lift}}$ from above, and learns a contextualized representation for the scene. Unlike the $\mathbf{PtC}_{\textrm{lift}}$ features which are local to just the object/mask or patch, we seek learned features that attend to different parts of the scene to obtain representations that capture the entire context of the scene. This is analogous to learning contextualized embeddings~\citep{Devlin2019BERT, Peters2018ELMO} as opposed to word-embeddings~\citep{Mikolov2013word2vec} in language. 

To learn such a representation, we take inspiration from the JEPA framework~\citep{Assran2023IJEPA, Bardes2024VJEPA} and develop 3D-JEPA. It is an encoder-predictor framework that performs masked prediction~\citep{He2021MAE,Devlin2019BERT} in the learned latent space. Concretely, let $\mathbf{PtC}$ be the input point cloud with some features (in our case, it contains lifted 2D foundation features). 3D-JEPA trains two transformer models $E_\theta(\cdot)$ and $P_\phi(\cdot)$ using the following objective,
\begin{equation}
    \min_{\theta, \phi} \ \  \Big|\Big| P_\phi \left( E_\theta(\mathbf{\tilde{PtC}}), M \right) - \mathrm{sg}\left( \bar{E}_\theta (\mathbf{PtC}) \right) \Big|\Big|,
\end{equation}
where $\tilde{\mathbf{Ptc}}$ denotes a masked view of the point cloud, $M$ is a mask variable describing regions that were masked, and $\mathrm{sg}(\cdot)$ is the stop-grad operator. Finally, $\bar{E}_\theta(\cdot)$ is the exponentiated moving average version of the encoder, which is important to prevent the representation from collapsing. Finally, the norm in this case is applied over each point in the masked subset of the point cloud. After training, $E_\theta(\cdot)$ is used as the contextualized representation.

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{assets/JEPA alg illustration.png}
    \caption{\textbf{Overview of the 3D-JEPA training framework.} The context encoder processes a masked point cloud to compute latent embeddings (per-point) that are context aware. Subsequently, a predictor operates on these latent embeddings to predict the embeddings of the masked regions. The target encoder has the same architecture as context encoder with weights being an exponentiated moving average over the course of training. The loss is computed per point in the embedding space and averaged across all the points that were masked.}
    \label{fig:enter-label}
\end{figure}

We note that we choose to perform masked prediction in latent space instead of the ambient/input space for two reasons. Firstly, unlike standard MAE used in 2D vision, our input space is high-dimensional. In fact, since we use lifted 2D foundation features, our input dimension is equivalent to feature dimension in ViT. We found directly reconstructing such fine-grained and high-dimensional features to be difficult. Secondly, in recent literature, methods that leverage masked prediction in teacher-student frameworks have produced the strongest results~\citep{Assran2023IJEPA, Oquab2023DINOv2}.

\paragraph{\bf Model Architectures}  Unlike images or voxels that contain a regular grid structure, point clouds are order invariant and set-valued. U-Net~\citep{iek20163DUnet}, PointNet~\citep{Qi2016PointNetDL} DeepSets~\citep{Zaheer2017DeepSets} and PointTransformer~\citep{Engel2020PointTransformer} have all emerged as promising architectures for point clouds. For our implementation of 3D-JEPA, we use PTv3~\citep{Wu2023PointTransformerV3} for the encoder. In each layer, it first serializes the point cloud based on local proximity using bijective space filling curves. Subsequently, points are grouped together and they attend to each other within the group, which is loosely analogous to convolutions. For the predictor, we use a similar serialization step, but then use a standard transformer with sparse attention pattern. This allows for faster mixing of information from the start, due to lack of an explicit grouping. However, we found sparse attention to be crucial for training throughput and memory, as well as for training stability. See appendix for further details about the architecture.

\paragraph{\bf Masking Patterns} We found the choice of masking pattern to play a crucial role in the quality of representations learned, consistent with prior literature in JEPA~\citep{Assran2023IJEPA, Bardes2024VJEPA}. In particular, among the variants we tried, the serialized percent masking pattern shown in Figure~\ref{fig:masking_patterns} to work the best. It contains two salient components: (1) masking out "regions" (points close in proximity) instead of random points, which can encourage better spatial understanding than simple local interpolation; and (2) masking out a percent of the scene instead of a fixed size, which allows for training on point clouds of varying spatial sizes.

\subsection{Language-conditioned 3D Mask and Bounding Box Decoder}
We employ a 3D decoder head that processes both featurized point cloud representations from 3D-JEPA and language queries to generate instance masks, bounding boxes, and text-to-prediction correspondence scores as seen in \cref{fig:3d_mask_decoder}. The architecture leverages a transformer decoder that follows the design of \cite{rodin}, integrating 3D-JEPA contextualized scene features and language queries alongside learnable object queries as showcased in \cref{fig:3d_transformer}. The transformer's refined features flow into parallel prediction heads for mask and bounding box regression.

\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{assets/3d_decoder.jpg}
    \caption{\centering Our Language-conditioned Mask and Bounding Box Decoder}
    \label{fig:3d_mask_decoder}
\end{figure}

\paragraph{\bf Prediction Heads} Our architecture consists of three parallel prediction heads. The mask head follows \cite{cheng2021maskformer} approach, using MLP-processed queries and computing dot products with point features to predict per-point mask logits. The text alignment head employs an MLP to ground predictions to specific noun-phrases in the query. For bounding boxes, we developed a novel architecture that explicitly concatenates linearly projected $x,y,z$ coordinates with point cloud features before doing a cross-attention operation with queries and before bounding box regression, as we found standard positional embeddings insufficient for accurate coordinate regression -- see \cref{fig:bbox_head} for a detailed diagram of the head.

\paragraph{\bf Joint Bounding box and Mask Supervision} While mask prediction alone achieves reasonable MaskIoU scores, extracting accurate bounding boxes from these masks proved challenging due to sensor noise issues (particularly around mirrors, windows, and RGB-D misalignment). We explored post-processing approaches like DBSCAN but found them unsatisfactory due to lower performance compared to our dedicated bounding box architecture and poor generalization in out-of-distribution scenarios. Conversely, training solely for bounding box regression without mask supervision proved extremely difficult, achieving less than $5\%$ accuracy due to the sparse nature of box supervision compared to dense mask supervision. Our final design jointly predicts masks and boxes, leveraging dense mask supervision for rich semantic understanding while using explicit box supervision to enforce spatial constraints. This joint approach achieves a $4\%$ absolute improvement in box IoU compared to mask-supervision with DBSCAN postprocessing while remaining fully differentiable, and it addresses the optimization challenges faced when training the box head in isolation.

\subsection{Training LocateX}

LocateX is trained using a combination of mask, box, and alignment losses, with Hungarian Matching to assign predictions to ground truth objects \cite{carion2020endtoendobjectdetectiontransformers}. We employ deep supervision with a weighted scheme where deeper decoder layers receive progressively higher weights, balancing training stability with model performance. The model is optimized using AdamW with with gradient clipping and an Exponential Moving Average (EMA) model for evaluation/inference. 

Fine-tuning the pretrained 3D-JEPA encoder requires careful scheduling to prevent training collapse. Our strategy employs separate warmup periods and learning rates for encoder and decoder components, with the encoder initially frozen during decoder warmup. The encoder maintains a lower learning rate relative to the decoder throughout training, with both components following an annealing schedule.

A key challenge in training LocateX is supervising a model operating on noisy sensor data using ScanNet annotations, which are on clean meshes. We transfer mesh annotations to sensor pointclouds by assigning each sensed point the distance-weighted average of ground truth labels from its k-nearest neighbors in the mesh. This supervision approach outperformed the alternative strategy of transferring predictions to the mesh space for supervision by ~6\%, as it ensures the model learns to handle all sensor points, including noise and artifacts crucial for real-world deployment.

\subsection{LocateX Model Card}
We opensource a model trained with the aforementioned components, and we evaluate its performance in Section~\ref{sec:experiments}. We opensource two components (1) The pre-trained Jepa PTV3 encoder and (2) LocateX with the JEPA encoder and localization head finetuned for 3D-RefExp.

\textbf{3D-JEPA backbone} The backbone is trained on ScanNet and ARKit [cite]. For pre-processing, we used SAM-H and CLIP-L + DINO-v2 [cites] for 2D foundation features. The encoder is a $\approx\mathbf{250}$ million parameter PT-v3 model with a feature dimension of $128$. We train the model with the serialized percent masking pattern depicted in Figure~\ref{fig:masking_patterns}. 

\textbf{LocateX:} We train our localization decoder from scratch and fine-tune the 3D-JEPA pretrained backbone. Our model is trained jointly across several referring expression benchmarks. Specifically, we train and evaluate on the 3D referential grounding datasets of SR3D, NR3D \citep{Achlioptas2020ReferIt3DNL} and ScanRefer \citep{chen2020scanrefer}. LocateX has $\approx\mathbf{580}$ million parameters. 


==> sections_ICML_sub/impact_statement.tex <==
\section*{Impact Statement}
\label{sec:impact}


This paper presents work whose goal is to advance the field of Machine Learning. There are many potential societal consequences of our work, none which we feel must be specifically highlighted here.

==> tables/ood.tex <==
\begin{table*}[ht]
    \centering
    \caption{\textbf{Performance on the three new evaluation datasets in LX3D.}
    We report accuracy @25 IoU.
    $^*$The GPT-4o VLM-Baseline was evaluated on 2,000 samples for SN++.
    \todo[inline]{Sergio/Ada update after all evals run}
    \todo[inline]{Decide on including FRE and FRE (chunked avg)}
    }
    \label{table:ood}
    \vspace*{5pt}
    \renewcommand{\arraystretch}{1.1}
    \begin{tabular}{l@{\hspace{8pt}}l@{\hspace{8pt}}lcccc}
        \toprule
        \multicolumn{3}{l}{} & SN++ & ARKitScenes & FRE & FRE (chunked avg) \\
        \multicolumn{3}{l}{\textit{Baselines}} \\
        \cmidrule(lr){1-7}
        \multicolumn{3}{l}{GPT-4o VLM-Baseline} & 60.5$^*$ & 21.6 & 18.9 & 40.3 \\
        \multicolumn{3}{l}{ConceptFusion + 3D-Decoder} & 47.0 & 22.0 & 1.0 & 51.3 \\
        \midrule
        \multicolumn{7}{l}{\textit{Ablations of \coolname{} and \coolname{}+}} \\
        \cmidrule(lr){1-3}
        Inputs & Encoder Init. & Finetuning Data & \multicolumn{4}{c}{} \\
        \cmidrule(lr){1-7}
        RGB & Random & SN & 35.0 & 11.0 & 13.0 & 31.0 \\
        CF & Random & SN & 50.0 & 42.0 & 28.0 & 53.7 \\
        CF & Random & SN + LX3D & 75 & 55 & -- & -- \\
        \midrule
        \multicolumn{7}{l}{\textit{\coolname{} and \coolname{}+ (ours)}} \\
        \cmidrule(lr){1-3}
        Inputs & Encoder Init. & Finetuning Data & \multicolumn{4}{c}{} \\
        \cmidrule(lr){1-7}
        CF & 3D-JEPA & SN & 54.0 & 47.0 & 25.0 & 61.7 \\
        CF & 3D-JEPA & SN + LX3D & \textbf{83.9} & \textbf{57.6} & \textbf{41.8} & \textbf{73.5} \\
        \bottomrule
    \end{tabular}
\end{table*}

==> tables/ood_short_errorbars.tex <==
\begin{table}[t]
    \centering
    \caption{
    \footnotesize
    \textbf{Generalization of \coolname{}.}
    We report accuracy @25 IoU. 
    % The ARKitScenes column contains both pretrain and val split as all models obtained the same results on either. 
    Using lifted 2D foundation features consistently improves results compared to RGB features, and 3D-JEPA pretraining further bolsters generalization.
    $^*$GPT-4o VLM-Baseline evaluated on 2,000 samples SN++ and 6,000 samples for SN Joint.
    }
    \label{table:ood_short}
    \vspace*{5pt}
    \resizebox{\linewidth}{!}{%
    \renewcommand{\arraystretch}{1.05}
    \newcommand{\colorone}{\cellcolor{green!5}}
    \newcommand{\colortwo}{\cellcolor{blue!15}}
    \begin{tabular}{@{}lcccc@{}}
        \toprule
        \textbf{Method} & \multicolumn{4}{c}{\textbf{Evaluation Dataset}} \\
        \midrule
        & \multicolumn{1}{c}{\colorone \textbf{ScanNet}} & \multicolumn{3}{c}{\colortwo\textbf{LX3D}} \\
        & \textbf{Joint Eval} &  \textbf{SN++} & \textbf{ARKitScenes} & \textbf{FRE} \\
        \midrule
        \rowcolor{gray!20} \multicolumn{5}{@{}l}{\textbf{Baselines}} \\
        GPT-4o VLM & 37.6 ± 0.63$^*$ & \textbf{60.5 ± 1.09}$^*$ & 26.8 ± 1.18 & 18.9 ± 1.93 \\
        CF + 3D-Decoder & 53.8 ± 0.27\phantom{$^*$} & 46.1 ± 0.75\phantom{$^*$} & 21.8 ± 1.10 & 48.9 ± 2.46 \\
        % \midrule
        \rowcolor{gray!20} \multicolumn{5}{@{}l}{\textbf{Ablations}} \\
        RGB, Random, SN & 51.3 ± 0.27\phantom{$^*$} & 37.5 ± 0.72\phantom{$^*$} & 11.3 ± 0.84 & 39.9 ± 2.41 \\
        CF, Random, SN & 58.8 ± 0.27\phantom{$^*$} & 51.5 ± 0.75\phantom{$^*$} & 41.7 ± 1.31 & \textbf{54.1 ± 2.46} \\
        % \midrule
        \rowcolor{gray!20} \multicolumn{5}{@{}l}{\textbf{Ours}} \\
        \coolname{} & \textbf{61.7 ± 0.26}\phantom{$^*$} & 56.7 ± 0.74\phantom{$^*$} & \textbf{46.2 ± 1.32} & 52.0 ± 2.46 \\
        \bottomrule
    \end{tabular}%
    }
\end{table}



